Large Scale Legal Text Classification Using Transformer Models

Large multi-label text classification is a challenging Natural Language Processing (NLP) problem that is concerned with text classification for datasets with thousands of labels. We tackle this problem in the legal domain, where datasets, such as JRC-Acquis and EURLEX57K labeled with the EuroVoc vocabulary were created within the legal information systems of the European Union. The EuroVoc taxonomy includes around 7000 concepts. In this work, we study the performance of various recent transformer-based models in combination with strategies such as generative pretraining, gradual unfreezing and discriminative learning rates in order to reach competitive classification performance, and present new state-of-the-art results of 0.661 (F1) for JRC-Acquis and 0.754 for EURLEX57K. Furthermore, we quantify the impact of individual steps, such as language model fine-tuning or gradual unfreezing in an ablation study, and provide reference dataset splits created with an iterative stratification algorithm.

==> README <==

November 21, 2012

IEEEtran.cls version 1.8 revises format specifications so that the final
layout more closely matches the layout of the Microsoft Word templates.

Additionally, the IEEEtran_HOWTO.pdf now includes the notice to not use
symbols, special characters, or math in the paper title and abstract.


*******


March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:  http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> reviews_comments.tex <==
== reviewer 1 ==

     The authors explore the performance of various recent transformer-based models in combination with strategies such as generative pretraining, gradual unfreezing and discriminative learning rates in order to reach competitive classification performance, and present new state-of-the-art results of 0.661 (F1) for JRC-Acquis and 0.754 for EURLEX57K. The study is interesting and relevant for the conference. The study is clearly presented, the paper well structure and the results justified.

----------------------

== reviewer 2 ==


This paper presents an extensive experimental evaluation comparing the performance of different transformer models in the context of large-scale legal text classification.
From my point of view, the experimental evaluation performed, and the fact that the authors are going to release the source code and the intermediate datasets generated, are valuable contributions.

It would be relevant to end Section II "RELATED WORK" with a conclusion and/or description of the research gaps that need to be covered, to properly motivate the research work proposed in the paper.

Zein: TODO 
// think about what to include?!


Add an evaluation of the computational costs (e.g., latencies) of the methods compared.
Zein: added at the end of discussion part

The authors indicate that it was not possible to fine-tune the LM on XLNet due to hardware constraints, but the hardware used has not been described. Please do it.
Zein: Add new section in V.A. Evaluation setup

Instead of using so many footnotes (some of which contain the same text, such as in the case of footnote 1 and footnote 7), please consider the possibility to use bibliographic references.
!!authors comment: fixed


Please, verify the URL provided in footnote 14. A character seems to be missing. 
!!authors comment: fixed

Please, revise the title of the paper in reference [21] (a strange character appears). 
!!authors comment: fixed


Some examples of typos: "is higher than of", "( [6])" (extra whitespace), "of dataset" should be replaced by "of the dataset", "of the first text A,then a" should be replaced by "of the first text A, then a".
!!authors comment: fixed


----------------

== reviewer 3 ==

In this paper, the authors present a study evaluating the performance of various transformer-based models for multi-label text classification using large-scale legal-domain corpora.


* Formatting


The paper is overall properly formatted with minor irregularities. (For example, note an extra empty line space after the subsection D. Transformer Models heading (p.5 left column) and a smaller space margin before the section VI. DISCUSSION heading (p.9 right column).)

ZEIN: CHECK AGAIN!

* Language


Overall the paper is readable and comprehensible and (relatively speaking, compared to more poorly-written papers) not too many grammatical errors or typos are noticed. Still, the authors are advised to review the suggestions at the end of feedback in order to correct errors and improve clarity.


* References


The number of references is appropriate for the type of paper. The references included are relevant to the content of the paper.


* Organization


The paper is properly organized, with appropriate division into sections and subsections.


* Presentation


The datasets, methodologies, and metrics used in the study and the results of evaluation are described in detail, and presented with the appropriate use of tables and figures.


* Relevance


The topic and content of the paper are relevant to the special track.


* Content


The quality of the technical content of the paper is acceptable.


* Questions


1.


“The advantages of using a multilingual and multi-domain thesaurus for document classification are manifold. Most importantly, it allows us to reduce the numbers of potential classes by going up the hierarchy which does not make classification incorrect but only more general. In this line, we use a class reduction method to generate datasets with a reduced number of classes by replacing the original labels with the top terms, microthesauri or domains they belong to.” (p.3 left column)


Would this not have the effect of generating overly general labels, thereby reducing the discriminatory efficacy of the labels when applied to multiple documents?

Zein: yes, that's true. We reduce the number of labels by generating general labels to show the efficiency of the models under different sets of labels. It is clear that the efficiency of the models will increase when discriminating between general labels.
Zein: section III.A was extended

2.


What could be the reason for the best performance by DistilBERT particularly for RP@1 and nDCG@1 (as shown in Table VI and Table VIII)?

Zein: RP@1 always equals to nDCG@1. 
// TODO: think about the reason. Actually, it is an interesting phenomena. and also it is the same in table VI (under different dataset). 
Zein: maybe we can not show a reason, but an observation.
- DistilBERT is more successful than roBERTa and BERT in retrieving the most probable label.
- RoBERTa is the best model in retrieving the most probable 3,5 labels. 
Zein: added to discussion

3.


In Table XII, why is there no case for 36 epochs with gradual unfreezing? Shouldn’t 0.645 Micro-F1 score be highlighted rather than 0.632 as the best score for DistilBERT? 

------------------------------------
Zein: The table was updated / corrected/ experiment redone.
Zein: The result of this experiment (36 without GU) was added.
----------------------------------------

4.


“… the effect of gradual unfreezing (GU), which for BERT has a large impact, with a relative improvement in F1 of about 6%” (p.9 right column)

Where does 6% come from (in Table XII)?

----------------------------------------------
Zein:
- The model "BERT without GU" resulted in Mic.F1 of 0.621, without GU Mic.F1 will improve to 0.661. so the improvement is 0.04/0.621 = 6%
----------------------------------------------------

* Suggestions on Language/Writing


“Text classification, that is the process of the assigning …” (p.1 left column)
-> Text classification, i.e., the process of assigning … 
!!authors comment: fixed


“In the later …” (p.1 left column)
-> In the latter … 
!!authors comment: fixed


“The around 7K terms …” (p.2 right column)
-> About 7K terms … 
!!authors comment: fixed


“… by going up the hierarchy which does not make classification incorrect ...” (p.3 left column)
-> by going up the hierarchy, which does not make classification incorrect … 
!!authors comment: fixed


“.. comprised of a many tables.” (p.3 right column)
-> … comprised of many tables. 
!!authors comment: fixed


“… higher than of the original descriptors.” (p.3 right column)
-> … higher than that of the original descriptors. 
!!authors comment: fixed


“The intuition is that in fine-turning … , that later layers …” (p.4 right column)
-> The intuition is that, in fine-tuning …, later layers … 
!!authors comment: fixed


“The F1-score is a common metric …, it is calculated …” (p.6 right column)
-> The F1-score is a common metric …, and it is calculated … 
!!authors comment: fixed


“Micro-F1 is an extension …, it treats …” (p.7 left column)
-> Micro-F1 is an extension …, and it treats … 
!!authors comment: fixed


“… predicting few relevant labels …” (p.7 left column)
-> … predicting a few relevant labels … 
!!authors comment: fixed


“The observations here as as follows …” (p.7 left column)
-> The observations here are as follows … 
!!authors comment: fixed


“… we run the experiments …” (p.7 right column)
-> … we ran the experiments … 
!!authors comment: fixed


“… strategy to optimizing performance.” (p.9 right column)
-> … strategy to optimize performance. (or … strategy for optimizing performance.) 
!!authors comment: fixed


“…, here we will summarize …” (p.9 right column)
-> …, so here we will summarize … 
!!authors comment: fixed

“… firstly we measured little differences between …” (p.9 right column)
-> … firstly we did not notice much difference between … 
!!authors comment: fixed

“…, it will be further studied …” (p.9 right column)
-> …, hence it will be further studied … 
!!authors comment: fixed

“…, firstly to potentially squeeze out higher performance …” (p.10 left column)
-> …, including potentially deriving higher performance … 
!!authors comment: fixed

--------------------

== reviewer 4 ==


The paper formatting needs some adjustments:


!! Eliminate all page numbers
!!authors comment: fixed


!! Capitalize the First Letter of each word in the title (not the conjunctions or prepositions);
!!authors comment: fixed


!! Correct the title; it is written using different font type and size – see template - Use 14 point Times New Roman in Bold

-------------------------------
Zein: I've used \Large with the title which is 14 points and bold. however, I am not sure if it is Times New Roman.
Erwin: just use the template with \title{}
-------------------------------------

!! add the author name & affiliation paragraph
!!authors comment: fixed

!! Keywords-text; text; text.
!! Correct punctuation
!!authors comment: fixed


!! avoid ALL the footnotes:
- if URLs, put them at References, refer to them via [x], and provide the date of the last access for ALL online references (see pages 1-6)
- if text only, embed them into the paper (see page 4)

----------------------------------
Zein: Adding links to reference is not nice, can we make an objection?
-------------------------------------

!! Insert Listing 1 as a numbered figure with caption; renumber all following figures

----------------------------------
Zein: Should I make a screenshot? better idea?
Erwin: i put the listing into a figure, moved the caption to the bottom and replace the reference within the text from "Listing" to "Figure". --> should be fine now
----------------------------------

!! Center all equations

!!authors comment: fixed

!! correct the format for all the References (see template):
- eliminate the indentation of all references
Zein: maybe fixed.

- list all the authors, if less than 6 [otherwise, use 'et al.' after the first author name] -> correct: [4], [11], [15], etc.

----------------------------
Zein: We are using their latex template! how could this happen! any idea how to fix it?
-------------------------------

- provide the last access date for ALL on-line references in the form [retrieved: month, year] (close to the camera-ready deadline) -> correct: [6], [8], [18], etc.

-----------------------------
Zein: I added ```urldate = {2020-09-01}``` to all of them but it didn't work, any idea how fix it?.
Erwin: change urldate to note, tried that for chalkidis2019large

------------------------------

!! Correct the format / grammar / punctuation errors. Some examples:
-- where datasets such as JRC-Acquis
Must be:
--> where datasets, such as JRC-Acquis
!!authors comment: example fixed


-- of individual
steps such as language
--> of individual steps, such as language
!!authors comment: fixed


-- In large multi-label text classification
(LMTC) the label space
--> In Large Multi-label Text Classification (LMTC), the label space
!! Apply this definition rule for all acronyms.
Zein: fixed for this example. will Check for similar cases

-- medical domain [2], [3],
--> medical domain [2][3],
Zein: fixed for this example. will Check for similar cases

-- In this work we focus on
--> In this work, we focus on
!! always this way, in similar constructions, across the whole paper
Zein: fixed for this example. will Check for similar cases

-- on different random splits which makes
--> on different random splits, which makes
!! across the entire paper, watch the rule of 'which', sometimes needing a ',' before
Zein: fixed for this example. will Check for similar cases


-- of related work in Section II we introduce
--> of related work in Section II, we introduce
!!authors comment: fixed

-- a new family of convolutional neural network
(CNN)
--> a new family of Convolutional Neural Network (CNN)
!!authors comment: fixed


-- In this paper we use the English
--> In this paper, we use the English
!!authors comment: fixed


-- dataset are similar ( [6]),
--> dataset are similar [6],
!!authors comment: fixed

!! etc., etc.

-----------------------

=======================
